Cosmological constraints on galaxy cluster structure

Observations of galaxy clusters (GC's) are a powerful tool to probe the evolution of the Universe at $z<2$. However, the determination of their real shape and structure is not completely understood and the assumption of asphericity is often used in several cosmological tests. In this work, we propose methods to infer the elongation of the gas distribution of GC's based on measurements of the cosmic expansion rate, luminosity distance to type Ia supernovae, X-Ray and Sunyaev-Zeldovich properties of GC's and on the validity of the so-called distance duality relation. For the sample considered, we find that the clusters look elongated preferentially aligned along the line of sight with the results of the different methods showing a good agreement with each other and with those predicted by the current cosmic concordance model.

==> table.tex <==
\tabletypesize{\scriptsize}
\def\arraystretch{1.0}
\begin{deluxetable}{lrr}
\tablecolumns{7}
\tablewidth{0pt}
\tablecaption{$e_{\rm l.o.s.}$}
\tablehead{
\colhead{Cluster}&\colhead{Method I }&\colhead{Method II}&\colhead{$\Lambda$CDM}  \\
}
\startdata
MS 1137.5+6625   &$1.57\pm{0.68}$  &$1.79\pm{0.68}$  &  \\ 
MS 0451.6-0305   &$0.80\pm{0.2}$   & $1.31\pm{0.11}$ & \\ 
Cl 0016+1609	   &$1.22\pm{0.30}$  & $1.49\pm{0.32}$ & \\
RXJ1347.5-1145   &$0.96\pm{0.23}$  &$1.45\pm{0.19}$  & \\
A 370            & $1.13\pm{0.47}$ & $1.81\pm{0.48}$ & \\ 
MS 1358.4+6245	 & $0.69\pm{0.20}$ & $1.40\pm{0.12}$ & \\ 
A 1995		       & $0.89\pm{0.22}$ & $1.24\pm{0.14}$ & \\ 
A 611		         & $1.02\pm{0.40}$ & $1.19\pm{0.27}$ & \\ 
A 697		         & $1.22\pm{0.35}$ & $1.67\pm{0.40}$ & \\ 
A 1835		       & $1.12\pm{0.19}$ & $1.43\pm{0.18}$ & \\ 
A 2261		       & $1.46\pm{0.40}$ & $1.54\pm{0.39}$ & \\ 
A 773		         & $1.96\pm{0.56}$ & $2.51\pm{0.71}$ & \\ 
A 2163		       & $1.13\pm{0.26}$ & $1.37\pm{0.23}$ & \\ 
A 520		         & $0.54\pm{0.22}$ & $1.77\pm{0.26}$ & \\ 
A 1689		       & $0.95\pm{0.13}$ & $1.14\pm{0.08}$ & \\ 
A 665		         & $0.69\pm{0.31}$ & $1.40\pm{0.29}$ & \\ 
A 2218		       & $1.30\pm{0.44}$ & $1.57\pm{0.45}$ & \\ 
A 1413		       & $0.89\pm{0.26}$ & $1.47\pm{0.20}$ & \\ 
A 2142		       & $0.90\pm{0.23}$ & $1.54\pm{0.18}$ & \\ 
A 478		         & $1.25\pm{0.55}$ & $1.95\pm{0.65}$ & \\ 
A 1651		       & $2.18\pm{1.21}$ & $2.71\pm{1.39}$ & \\ 
A 401		         & $1.20\pm{0.23}$ & $1.67\pm{0.27}$ & \\ 
A 399		         & $0.55\pm{0.18}$ & $1.71\pm{0.12}$ & \\ 
A 2256		       & $0.99\pm{0.28}$ & $1.38\pm{0.22}$ & \\ 
A 1656		       & $1.0\pm{0.45}$ & $1.23\pm{0.32}$ & \\
\enddata
\tablecomments{Cluster elongation along the l.o.s. and maximum axial ratio.}
\label{tab:3D_morph}
\end{deluxetable}
